Scene Understanding Enabled Semantic Communication with Open Channel Coding

As communication systems transition from symbol transmission to conveying meaningful information, sixth-generation (6G) networks emphasize semantic communication. This approach prioritizes high-level semantic information, improving robustness and reducing redundancy across modalities like text, speech, and images. However, traditional semantic communication faces limitations, including static coding strategies, poor generalization, and reliance on task-specific knowledge bases that hinder adaptability. To overcome these challenges, we propose a novel system combining scene understanding, Large Language Models (LLMs), and open channel coding, named \textbf{OpenSC}. Traditional systems rely on fixed domain-specific knowledge bases, limiting their ability to generalize. Our open channel coding approach leverages shared, publicly available knowledge, enabling flexible, adaptive encoding. This dynamic system reduces reliance on static task-specific data, enhancing adaptability across diverse tasks and environments. Additionally, we use scene graphs for structured semantic encoding, capturing object relationships and context to improve tasks like Visual Question Answering (VQA). Our approach selectively encodes key semantic elements, minimizing redundancy and improving transmission efficiency. Experimental results show significant improvements in both semantic understanding and efficiency, advancing the potential of adaptive, generalizable semantic communication in 6G networks.

==> ACM_Sys/name.tex <==
### Scene Understanding-Oriented LLM-Semantic Decoding

In this approach, we aim to enhance the accuracy and completeness of received data, which may be corrupted or incomplete due to transmission issues, by using large language models (LLMs). The key idea is to leverage the semantic knowledge embedded in structured data (such as scene graphs) to correct errors and supplement missing information, ensuring a more reliable and accurate representation of the data in a structured format, such as JSON. 

#### 1. Reconstruction of Initial Information

The first step involves the conversion of token IDs into readable text. This is done by using a tokenizer to map the numeric token IDs back to their corresponding textual tokens. The output of this step is the reconstructed initial information, which is expressed as:

\[
\mathbf{x} = [\text{initial\_information}_1, \ldots, \text{initial\_information}_n]
\]

Here, \( \mathbf{x} \) represents the sequence of tokens that, when mapped, form the initial information.

#### 2. Enhancement with Structured Information

The reconstructed information may be incomplete or contain errors, so we supplement it with previously structured knowledge. This structured information typically includes object attributes such as quantity, location, and relationships, and is organized in the form of a Scene Graph. The structured data is represented as:

\[
\mathbf{p} = [\text{previous\_information}_1, \ldots, \text{previous\_information}_m]
\]

This structured data provides additional context, allowing the LLM to correct and enrich the initial information.

#### 3. LLM-based Semantic Enhancement

The LLM is responsible for integrating the initial information with the structured data. The model processes both inputs, learning to generate a corrected and enriched version of the data. This process can be described as a series of operations through a multi-layer perceptron (MLP), where the inputs are processed in multiple hidden layers to produce the final output:

\[
\mathbf{h}_1 = \sigma(W_1 [\mathbf{x}; \mathbf{p}] + \mathbf{b}_1)
\]

Subsequent layers process this output iteratively:

\[
\mathbf{h}_L = \sigma(W_L \mathbf{h}_{L-1} + \mathbf{b}_L)
\]

Finally, the corrected and enhanced information is obtained as:

\[
\text{final\_information} = W_{\text{out}} \mathbf{h}_L + \mathbf{b}_{\text{out}}
\]

The output \( \text{final\_information} \) contains three key components: number, location, and relationship.

\[
\text{final\_information} = [n, l, r]
\]

Where \( n \) is the object count, \( l \) is the location, and \( r \) represents the relationships between objects.

#### 4. Conversion to JSON Format

The final enhanced information is converted into a structured JSON format for easy storage and further processing:

\[
\text{json\_data} = \left\{
\begin{array}{ll}
\text{"number"} & : n \\
\text{"location"} & : l \\
\text{"relationship"} & : r
\end{array}
\right\}
\]

This conversion allows for the data to be easily accessed and utilized in subsequent steps.

#### 5. Query Handling with Scene Graph Data

When a user query is received, it follows a similar process. The query is reconstructed and corrected using the LLM, then compared with the scene graph to extract relevant information such as object count, location, or relationships. The process is as follows:

1. Query Reconstruction: The LLM corrects and reconstructs the query from token IDs to a meaningful question.
2. Scene Graph Query: Based on the query, relevant structured data is retrieved from the scene graph.
3. Preliminary Answer Generation: The LLM uses the retrieved scene graph data to generate an initial response.
4. Enhanced Answer: The LLM integrates the context from the query and scene graph to provide a semantically enriched and accurate answer.

---

This approach ensures that transmission errors and missing information are effectively corrected, while enhancing the context of the data through structured scene graphs. By combining the power of LLMs and scene understanding, the system can provide more accurate, contextually relevant responses, making it suitable for complex tasks such as visual question answering (VQA) and semantic content generation.
